A Differential Effect Approach to Partial Identification of Treatment Effects

We consider identification and inference for the average treatment effect and heterogeneous treatment effect conditional on observable covariates in the presence of unmeasured confounding. Since point identification of these treatment effects is not achievable without strong assumptions, we obtain bounds on these treatment effects by leveraging differential effects, a tool that allows for using a second treatment to learn the effect of the first treatment. The differential effect is the effect of using one treatment in lieu of the other. We provide conditions under which differential treatment effects can be used to point identify or partially identify treatment effects. Under these conditions, we develop a flexible and easy-to-implement semi-parametric framework to estimate bounds and leverage a two-stage approach to conduct statistical inference on effects of interest. The proposed method is examined through a simulation study and a case study that investigates the effect of smoking on the blood level of cadmium using the National Health and Nutrition Examination Survey.

==> application.tex <==
\section{Case Study: Effectiveness of Right Heart Catheterization (RHC) in the Initial Care of Critically Ill Patients}
\label{sec: application RHC}
\subsection{Background, all samples and matched samples}
We apply our developed method and illustrate various aspects of it using an observational study investigating the effectiveness of right heart catheterization (RHC) in the initial care of critically ill patients. Since its introduction into the intensive care units (ICUs) almost $50$ years ago, RHC was perceived by clinicians as largely beneficial because direct measurements of heart function by RHC help guide therapies, which was believed to lead eventually to more favorable patient outcomes (\citealp{connors1983evaluation,connors1996effectiveness}). In fact, the belief in RHC's effectiveness was so strong that many physicians refused to enroll their patients into randomized controlled trials (RCTs) for ethical considerations (\citealp{guyatt1991randomized}). In the absence of RCTs, \citet{connors1996effectiveness} examined the effectiveness of RHC in a matching-based prospective cohort study using observational data. We followed \citet{rosenbaum2012optimal} and considered patients under the age of $65$ from the work of \citet{connors1996effectiveness}; among these patients there are $1194$ patients who received RHC and $1804$ who did not. We followed \citet{connors1996effectiveness} and considered observed covariates related to patients demographics, laboratory measurements and vital signs because these factors clearly affect both physicians' decision to use or withhold RHC and patients' outcomes. The primary outcome of interest is patients' 30-day mortality.

\begin{table}[ht]
\centering
\caption{\small Balance table of all samples and the matched samples. There are a total of $1194$ patients under $65$ undergoing RHC and $1804$ not undergoing RHC. A total of $1194$ matched pairs were formed. SMD is the abbreviation of the standardized mean difference.}
\label{tbl: balance table}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccc}
  \hline
 & \multirow{3}{*}{\begin{tabular}{c}All Samples \\RHC \\ ($n = 1194$)\end{tabular}}  & \multirow{3}{*}{\begin{tabular}{c}All Samples\\ No RHC\\ ($n = 1804$)\end{tabular}} & \multirow{3}{*}{\begin{tabular}{c}Absolute \\ SMD\end{tabular}} & \multirow{3}{*}{\begin{tabular}{c}Matched Samples\\ No RHC \\ ($n = 1194$)\end{tabular}} & \multirow{3}{*}{\begin{tabular}{c}Absolute \\ SMD\end{tabular}} \\ \\ \\
  \hline
  \textbf{Demographics} \\
  \hspace{0.3cm} Age, yr & 49.56 & 48.01 & 0.09 & 49.26 & 0.02 \\ 
  \hspace{0.3cm} Male, \% & 0.58 & 0.57 & 0.02 & 0.59 & 0.01 \\ 
  \hspace{0.3cm} White, \% & 0.72 & 0.72 & 0.01 & 0.73 & 0.02 \\ 
  \textbf{Laboratory Measurements} \\
  \hspace{0.3cm} PaO$_2$/FiO$_2$, mm Hg & 196.13 & 243.68 & 0.29 & 214.55 & 0.11 \\ 
  \hspace{0.3cm} PaO$_2$, mm Hg & 36.74 & 38.67 & 0.11 & 37.62 & 0.05 \\ 
  \hspace{0.3cm} WBC count, $\times 10^9$L & 15.77 & 14.98 & 0.05 & 15.29 & 0.03 \\ 
  \hspace{0.3cm} Creatinine, $\mu$mol/L & 2.46 & 1.94 & 0.17 & 2.15 & 0.10 \\ 
  \textbf{Vital Signs} \\
  \hspace{0.3cm} Blood pressure, mm Hg & 69.44 & 87.47 & 0.35 & 75.95 & 0.13 \\ 
  \hspace{0.3cm} APACHE III score & 61.07 & 50.51 & 0.36 & 55.63 & 0.19 \\ 
  \hspace{0.3cm} Coma score & 17.90 & 21.66 & 0.09 & 16.49 & 0.03 \\ 
  \textbf{Propensity Score} & 0.48 & 0.35 & 0.55 & 0.42 & 0.24 \\ 
   \hline
\end{tabular}}
\end{table}

The first three columns of Table \ref{tbl: balance table} summarize patient characteristics in the full sample. Not surprisingly, a number of important variables are vastly different between the two groups; for instance, the mean blood pressure is only $69.44$ mm Hg in the RHC group compared to $87.47$ mm Hg in the no RHC group. Overall, the two groups before matching have similar demographics but the RHC group was sicker. We adopt a matched-pair study design as in \citet{connors1996effectiveness} and \citet{rosenbaum2012optimal}, and form $1194$ matched pairs of two patients (one receiving RHC and the other not) using optimal matching (based on a robust version of the Mahalanobis distance) within a $0.2$ standard deviation propensity score caliper (\citealp{rosenbaum1985constructing,rosenbaum2002observational,rosenbaum2010design}). It is evident that after matching, observed covariates in the RHC and no RHC groups are much closer; however, the question remains as to whether they are ``close" enough to justify a randomization-based analysis of the primary outcome of 30-day mortality status.

\subsection{Testing the randomization assumption, residual sensitivity value and outcome analysis}
We applied our metric-learning-enhanced clustering algorithm to the matched sample to test Assumption \ref{assum: randomization inference}; the test statistic $t = |\Pi_1 \cap \mathcal{T}|$ equals $659$ and yields a $p$-value of $0.0004$, providing strong evidence that the randomization assumption may not hold for these $1194$ matched pairs. Next, we aimed to quantify the residual confounding due to observed covariates not well matched by testing Assumption \ref{assum: biased randomization inference} for assorted values of $\Gamma$. The first two columns of Table \ref{tbl: outcome analysis results} tabulate the $p$-values corresponding to testing Assumption \ref{assum: biased randomization inference} for each specified $\Gamma$ value, and suggest that the residual sensitivity value $\underline{\widetilde{\Gamma}}$ is approximately equal to $1.10$ for the matched samples. In other words, though a randomization assumption is not suitable for the matched samples, a slightly relaxed version with $\Gamma = 1.10$ is deemed plausible. In a supplementary analysis, we further considered $1194$ matched pairs formed using the propensity score matching and obtained a residual sensitivity value equal to $1.09$. For this particular real data example, the propensity score matching and optimal matching produced very similar covariate balance and residual sensitivity value. Either design may be used in the downstream outcome analysis.


The last two columns of Table \ref{tbl: outcome analysis results} summarize the outcome analysis $p$-values based on McNemar's test under the randomization assumption ($\Gamma = 1$) and the bounding $p$-values under Rosenbaum's sensitivity analysis framework corresponding to each $\Gamma > 1$, all against the alternative hypothesis that RHC has a negative effect on 30-day mortality; the outcome analysis and associated sensitivity analysis were performed using \textsf{R} package \textsf{rbounds} (\citealp{R_pkg_rbounds}). As suggested by Table \ref{tbl: outcome analysis results}, if one adopts the randomization assumption for these $1194$ matched pairs, one would report a $p$-value equal to $0.0220$ in the primary analysis and conclude that RHC has a negative effect on patients' 30-day mortality and this effect would go away when there is unmeasured confounding up to $\Gamma = 1.03$, roughly corresponding to an unmeasured confounder that simultaneously increases the odds of receiving RHC by $25\%$ and the odds of death by $30\%$ (\citealp{rosenbaum2009amplification}). On the other hand, if one uses our proposed procedure to first test the randomization assumption and take into account the residual sensitivity value $\underline{\Tilde{\Gamma}} = 1.10$ in the primary analysis, one would instead report the bounding $p$-value corresponding to taking $\Gamma = \underline{\Tilde{\Gamma}} = 1.10$ in the primary analysis and conclude that there is insufficient evidence against the null hypothesis of no effect.

\begin{table}[h]
    \centering
    \caption{\small The first two columns report the $p$-values testing the biased randomization assumption \ref{assum: biased randomization inference} for assorted $\Gamma$ values. The residual sensitivity value $\underline{\Tilde{\Gamma}}$ approximately equals $1.10$ for the matched samples. The third and fourth columns report the $p$-value of the outcome analysis under the randomization assumption $(\Gamma = 1.00)$ and bounding $p$-values in the associated sensitivity analyses $(\Gamma > 1)$. The outcome analysis is not significant when the residual sensitivity value is taken into account ($p$-value = $0.1714$ when $\Gamma = \underline{\Tilde{\Gamma}} = 1.10$). }
    \label{tbl: outcome analysis results}
    \begin{tabular}{ccccccc} \hline
        \multicolumn{3}{c}{\multirow{3}{*}{\begin{tabular}{c}Testing \\ Assumption \ref{assum: biased randomization inference}\end{tabular}}} & \multicolumn{2}c{\multirow{3}{*}{\begin{tabular}{c}Outcome \\ Analysis\end{tabular}}} \\ \\ \\
    $\Gamma = 1.00$ & 0.0004 & & $\Gamma = 1.00$ & 0.0220  \\
        $\Gamma = 1.02$ & 0.0012 & & $\Gamma = 1.02$ & 0.0366  \\
    $\Gamma = 1.04$ & 0.0036 & & $\boldsymbol{\Gamma = 1.03}$ & $\boldsymbol{0.0462}$  \\
    $\Gamma = 1.06$ & 0.0098 & & $\Gamma = 1.04$ & $0.0576$  \\
    $\Gamma = 1.08$ & $0.0237$ & &$\boldsymbol{\Gamma = 1.10}$ & $\boldsymbol{0.1714}$ \\
$\boldsymbol{\Gamma = 1.10}$ & $\boldsymbol{0.0517}$ & &$\Gamma = 1.20$ & 0.5087  \\ \hline
    \end{tabular}
\end{table}
